Accelerated and instance-optimal policy evaluation with linear function approximation

We study the problem of policy evaluation with linear function approximation and present efficient and practical algorithms that come with strong optimality guarantees. We begin by proving lower bounds that establish baselines on both the deterministic error and stochastic error in this problem. In particular, we prove an oracle complexity lower bound on the deterministic error in an instance-dependent norm associated with the stationary distribution of the transition kernel, and use the local asymptotic minimax machinery to prove an instance-dependent lower bound on the stochastic error in the i.i.d. observation model. Existing algorithms fail to match at least one of these lower bounds: To illustrate, we analyze a variance-reduced variant of temporal difference learning, showing in particular that it fails to achieve the oracle complexity lower bound. To remedy this issue, we develop an accelerated, variance-reduced fast temporal difference algorithm (VRFTD) that simultaneously matches both lower bounds and attains a strong notion of instance-optimality. Finally, we extend the VRFTD algorithm to the setting with Markovian observations, and provide instance-dependent convergence results. Our theoretical guarantees of optimality are corroborated by numerical experiments.

==> command-template.tex <==
%!TEX root = main-paper-template.tex

% The command above makes the PDF compilable from this file if you're using SublimeText

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Some basic packages

\usepackage{comment}
\usepackage{epsf}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{bbm}
\usepackage{color}
\usepackage{nicefrac}
\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{amsmath, bm}
\usepackage{amssymb}
\usepackage{textcomp}
\usepackage{xcolor}
%\usepackage[ruled, vlined, lined, commentsnumbered]{algorithm2e}
\usepackage{algorithm,algorithmic}

\RequirePackage[colorlinks,citecolor={blue!60!black},urlcolor={blue!70!black},linkcolor={red!60!black},breaklinks,hypertexnames=false]{hyperref} %Adds links to references (without boxes)


% Alternative minipage environment, renders better in terms of spacing

\newenvironment{fminipage}%
  {\begin{Sbox}\begin{minipage}}%
  {\end{minipage}\end{Sbox}\fbox{\TheSbox}}
  
\newenvironment{algbox}[0]{\vskip 0.2in
\noindent 
\begin{fminipage}{6.3in}
}{
\end{fminipage}
\vskip 0.2in
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MACROS BELOW

%%%%%%%

% {Theorem, Proposition, Lemma, Corollary} numbered sequentially
% throughout the paper, not by section number and not combined


\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{conjecture}{Conjecture}
\newtheorem{claim}{Claim}

%%%%%%%%%%%
%References (natbib): Use \citet and \citep to take full advantage

\usepackage{natbib}
\setcitestyle{round}

%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Widebar command
\newlength{\widebarargwidth}
\newlength{\widebarargheight}
\newlength{\widebarargdepth}
\DeclareRobustCommand{\widebar}[1]{%
 \settowidth{\widebarargwidth}{\ensuremath{#1}}%
 \settoheight{\widebarargheight}{\ensuremath{#1}}%
 \settodepth{\widebarargdepth}{\ensuremath{#1}}%
 \addtolength{\widebarargwidth}{-0.3\widebarargheight}%
 \addtolength{\widebarargwidth}{-0.3\widebarargdepth}%
 \makebox[0pt][l]{\hspace{0.3\widebarargheight}%
   \hspace{0.3\widebarargdepth}%
   \addtolength{\widebarargheight}{0.3ex}%
   \rule[\widebarargheight]{0.95\widebarargwidth}{0.1ex}}%
 {#1}}



%%% New version of \caption puts things in smaller type, single-spaced 
%%% and indents them to set them off more from the text.
\makeatletter
\long\def\@makecaption#1#2{
       \vskip 0.8ex
       \setbox\@tempboxa\hbox{\small {\bf #1:} #2}
       \parindent 1.5em 
       \dimen0=\hsize
       \advance\dimen0 by -3em
       \ifdim \wd\@tempboxa >\dimen0
               \hbox to \hsize{
                       \parindent 0em
                       \hfil 
                       \parbox{\dimen0}{\def\baselinestretch{0.96}\small
                               {\bf #1.} #2
                               %%\unhbox\@tempboxa
                               } 
                       \hfil}
       \else \hbox to \hsize{\hfil \box\@tempboxa \hfil}
       \fi
       }
\makeatother



%% COMMENTING commands: insert more for more than two collaborators

\long\def\comment#1{}

\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\black}[1]{\textcolor{black}{#1}}
\newcommand{\apcomment}[1]{{\bf{{\blue{{AP --- #1}}}}}}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\mycomment}[1]{{\bf{{\red{{TL --- #1}}}}}}



% Some vector/matrix norms. Convention is that we use triple lines for matrix 
% norms and double lines for vector norms.
\newcommand{\matnorm}[3]{|\!|\!| #1 | \! | \!|_{{#2}, {#3}}}
\newcommand{\matsnorm}[2]{|\!|\!| #1 | \! | \!|_{{#2}}}
\newcommand{\vecnorm}[2]{\| #1\|_{#2}}

% Some useful and common operators
% Independence symbol
\newcommand\indpt{\protect\mathpalette{\protect\independenT}{\perp}} 
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\defn}{\coloneqq} %This is a properly aligned definition symbol
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator{\modd}{mod}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Var}{var}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator{\floor}{floor}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\range}{range}
\DeclareMathOperator{\dist}{\rho}



% Specific norms
\newcommand{\nucnorm}[1]{\ensuremath{\matsnorm{#1}{\footnotesize{\mbox{nuc}}}}}
\newcommand{\fronorm}[1]{\ensuremath{\matsnorm{#1}{\tiny{\mbox{F}}}}}
\newcommand{\opnorm}[1]{\ensuremath{\matsnorm{#1}{\tiny{\mbox{op}}}}}
\newcommand{\eucnorm}[1]{\left\|#1 \right\|}
\newcommand{\linfnorm}[1]{\left\|#1 \right\|_\infty}

% Bracket notation to make life easier when writing long expressions
\newcommand{\paren}[1]{\left\{ #1 \right\} }
% Inner product
\newcommand{\inprod}[2]{\ensuremath{\langle #1 , \, #2 \rangle}}
\newcommand{\inprodpi}[2]{\ensuremath{\langle #1 ,  #2 \rangle_\Pi}}

% The macros below are useful if you see these quantities changing over the course of writing
\newcommand{\numdim}{\ensuremath{d}}
\newcommand{\numobs}{\ensuremath{n}}

% Distances between distributions
\newcommand{\kull}[2]{\ensuremath{D_{\mathsf{KL}}(#1\; \| \; #2)}}
\newcommand{\KL}{\ensuremath{D_{\mathsf{KL}}}}
\newcommand{\TV}{\ensuremath{d_{\mathsf{TV}}}}
\newcommand{\Hel}{\ensuremath{d_{\mathsf{hel}}}}

% Probability
\newcommand{\EE}{\ensuremath{{\mathbb{E}}}}
\newcommand{\Prob}{\ensuremath{{\mathbb{P}}}}
\newcommand{\ind}[1]{\ensuremath{{\mathbb{I}\left\{ #1 \right\}}}}

%Numbering (use with \overset to label steps)
\newcommand{\1}{\ensuremath{{\sf (i)}}}
\newcommand{\2}{\ensuremath{{\sf (ii)}}}
\newcommand{\3}{\ensuremath{{\sf (iii)}}}
\newcommand{\4}{\ensuremath{{\sf (iv)}}}
\newcommand{\5}{\ensuremath{{\sf (v)}}}
\newcommand{\6}{\ensuremath{{\sf (vi)}}}

%Eigenvector / eigenvalue related notation
\newcommand{\eig}[1]{\ensuremath{\lambda_{#1}}}
\newcommand{\eigmax}{\ensuremath{\eig{\max}}}
\newcommand{\eigmin}{\ensuremath{\eig{\min}}}


% Distributions
\newcommand{\NORMAL}{\ensuremath{\mathcal{N}}}
\newcommand{\BER}{\ensuremath{\mbox{\sf Ber}}}
\newcommand{\BIN}{\ensuremath{\mbox{\sf Bin}}}
\newcommand{\Hyp}{\ensuremath{\mbox{\sf Hyp}}}

% Script letters
\newcommand{\Aspace}{\ensuremath{\mathcal{A}}}
\newcommand{\Xspace}{\ensuremath{\mathcal{X}}}
\newcommand{\Yspace}{\ensuremath{\mathcal{Y}}}
\newcommand{\Zspace}{\ensuremath{\mathcal{Z}}}
\newcommand{\Fspace}{\ensuremath{\mathcal{F}}}

% Population and sample loss functions
\newcommand{\loss}{\ensuremath{\mathcal{L}}}
\newcommand{\lossn}[1]{\ensuremath{\mathcal{L}^n \left( #1 \right)}}

% True parameter
\newcommand{\thetastar}{\ensuremath{\theta^*}}
% Estimates
\newcommand{\thetahat}{\ensuremath{\widehat{\theta}}}
\newcommand{\thetabar}{\ensuremath{\overline{\theta}}}
\newcommand{\thetatil}{\ensuremath{\widetilde{\theta}}}

% Order notation
\newcommand{\order}{\ensuremath{\mathcal{O}}}
\newcommand{\ordertil}{\ensuremath{\widetilde{\order}}}
\newcommand{\Omegatil}{\ensuremath{\widetilde{\Omega}}}

% Notations by Tianjiao
\newcommand{\vbar}{\ensuremath{\bar v}}
\newcommand{\skipcon}{C_P}
\newcommand{\mixcon}{C_M}
\newcommand{\param}{\vartheta}





\def\dist{\mathrm{dist}}
\def\prox{\mathrm{prox}}
\def\proj#1{\Pi_{X^n}^{\psi}\left(#1\right)}
\def\a{\alpha}
\def\b{\beta}
\def\e{\epsilon}
\def\d{\delta}
\def\g{\gamma}
\def\t{\theta}
\def\o{\omega}
\def\s{\sigma}
\def\l{\lambda}
\def\n{\nabla}
\def\wh{\widehat}
\def\wt{\widetilde}
\def\tsy{\textstyle}
\newcommand{\tsum}{\textstyle{\sum}}
\def\sm{\textstyle{\tfrac{1}{m}\sum_{i=1}^m}}
\def\smn{\textstyle{\sum}_{i=1}^m}
\def\sk{\textstyle{\sum}_{t=1}^s}
\def\skt{\textstyle{\sum}_{t=2}^s}
\def\sl{\textstyle{\sum}_{\ell=1}^k}
\def\sll{\textstyle{\sum}_{\ell=2}^k}
\def\slk{\textstyle{\sum}_{\ell=1}^{k-1}}
\def\dtb{\boldsymbol{\d}}
\def\R{\mathbb{R}}
\def\M{\mathcal{M}}
\def\O{\mathcal{O}}
\def\la{\langle}
\def\ra{\rangle}
\def\lla{\left\langle}
\def\rra{\right\rangle}
\def\ux{\underline{x}}
\def\ty{\widetilde{y}}
\def\bx{\bar{x}}
\def\Bx{{\textbf{x}}}
\def\bBx{\bar{\textbf{x}}}
\def\eBx{\emph{\textbf{x}}}
\def\by{\bar{y}}
\def\l{\ell}
\def\lbd{\lambda}
\def\Eb{\mathbb{E}}
\def\lc{\left\lceil}   
\def\rc{\right\rceil}


\def\bfA{\mathbf{A}}
\def\bfb{\mathbf{b}}

\def\eqnok#1{(\ref{#1})}
\usepackage{epsfig}
\usepackage{calc}
\usepackage{amstext}
\usepackage{amsmath}
\usepackage{multicol}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{bm}
\usepackage{xcolor}
\usepackage{comment}
\usepackage[scientific-notation=true]{siunitx}

\newcommand{\AR}[2]{\left[\begin{array}{#1}#2\end{array}\right]}
\newcommand{\gk}[2]{{\scriptsize\color{red}}{\color{green}\  #2}}
\newcommand{\gl}[2]{{\scriptsize\color{red}}{\color{green}\  #2}}
\newcommand{\tl}[2]{{\scriptsize\color{red}}{\color{green}\  #2}}
\newcommand{\trace}{\mathrm{trace}}
%\newcommand{\diag}{\mathrm{diag}}
\newcommand{\rand}{\mathrm{rand}}
%\newcommand{\rank}{\mathrm{rank}}
\newcommand{\T}{\mathrm{T}}
\newcommand{\SDP}{\mathrm{SDP}}
\newcommand{\Lin}{\mathrm{Lin}}
\newcommand{\OPT}{\mathrm{OPT}}
\newcommand{\gap}{\mathrm{gap}}
\newcommand{\res}{\mathrm{res}}
\newcommand{\erf}{\mathrm{erf}}
\newcommand{\todo}[1]{\vspace{5 mm}\par \noindent \marginpar{\textsc{ToDo}}
	\framebox{\begin{minipage}[c]{0.95 \columnwidth} \tt #1
	\end{minipage}}\vspace{5 mm}\par }
\newcommand{\tmix}{t_{\mathsf{mix}}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\MarkovS}{\bar{\Sigma}_{\mathsf{Mkv}}}
\newcommand{\iidS}{\bar{\Sigma}_{\mathsf{iid}}}



\newcommand{\bbr}{\Bbb{R}}
\newcommand{\beq}{\begin{equation}}
	\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
	\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\beqas}{\begin{eqnarray*}}
	\newcommand{\eeqas}{\end{eqnarray*}}

%\usepackage{algorithm,algorithmic}
\usepackage{bbm}
\def\argmin{{\rm argmin}}
\def\argmax{{\rm argmax}}
\def\Argmax{{\rm Argmax}}
\def\Argmin{{\rm Argmin}}
\def\bbe{{\mathbb{E}}}
\def\bbs{{\mathbb{S}}}
\def\bbx{{\mathbb{X}}}
\def\vgap{\vspace*{.1in}}
\newcommand{\nn}{\nonumber}
